Speech Emotion Recognition with ASR Integration

Speech Emotion Recognition (SER) plays a pivotal role in understanding human communication, enabling emotionally intelligent systems, and serving as a fundamental component in the development of Artificial General Intelligence (AGI). However, deploying SER in real-world, spontaneous, and low-resource scenarios remains a significant challenge due to the complexity of emotional expression and the limitations of current speech and language technologies. This thesis investigates the integration of Automatic Speech Recognition (ASR) into SER, with the goal of enhancing the robustness, scalability, and practical applicability of emotion recognition from spoken language.

==> edengfmt.tex <==
%%
%% edengfmt.tex - User defined formatting for thesis class
%%
%% Copyright (C) 2010-2018 Mathew Topper <damm_horse@yahoo.co.uk>
%%
%%   ABOUT
%%
%% This is the user defined formatting file for a Latex2e template which
%% corresponds to the regulations regarding layout of a thesis submitted within
%% the University of Edinburgh. 
%%
%% IN THIS FILE YOU CAN:
%%
%%   ** SET THE MARGINS
%%   ** SET THE LINE SPACING
%%   ** CONTROL THE HYPHENATION
%%   ** ADD VERTICAL SPACE IN ALIGNED EQUATIONS
%%   ** FORMAT THE TABLE OF CONTENTS AND LISTS
%%   ** FORMAT THE BIBLIOGRAPHY
%%   ** CHANGE FONT SIZE OF SUBFIGURE CAPTIONS
%%   ** HYPERREF SETTINGS
%%   ** FORMAT FANCY HEADERS
%%   ** FIX VBOX ERROR WITH 'twoside' OPTION

%%%% SET THE MARGINS

%% Note, the margins here are University of Edinburgh, School of Engineering
%% regulation. You may wish to borrow a millimetre here or there and change
%% the header, for example, and thus the setting of the margins has been made
%% available here. It's not recommended you change these too much!
%% Note: Margins are controlled by the 'geometry' package.
\geometry{top=20mm, inner=40mm, outer=25mm, bottom=40mm}

%% Control the header height and separation for fancyhdr
\geometry{headheight=15.2pt, headsep=4mm}

%% Set the space between the main text and the start of the footnone
\geometry{footnotesep=5mm}

%% Set the space to the footer. We need to define a new length before applying
%% it in order to use the minus rubber length to aid flexibility.
\newlength\myfootskip
\setlength\myfootskip{20mm minus 1em}

\geometry{footskip=\myfootskip}


%%%% SET THE LINE SPACING.

%% Controlled by `setspace' package.
%% Note: you can define environments for different spacings during the
%% document, ie \begin{singlespace}blah blah\end{singlespace}.
%%
%% Quotes are automatically single spaced via this method.

%% Pick one of these three options for global spacing.

% \singlespacing                       % Single spaced

\onehalfspacing                        % One and a half spaced

% \doublespacing                       % Double spacing

% \setstretch{1.45}                    % Custom spacing. 1.3 ~ onehalf &
                                       % 1.6 ~ double spaced

%%%% HYPHENATION

%% The university regs say ``hyphenation should be avoided if possible''.
%% Latex looks rubbish with no hypenation but you can discourage it until
%% you start to get lots of bad boxs. Try to set this number as high as
%% possible (0-10000). You can also set a separate value for the
%% bibliography using \bibhyphenpenalty.
\hyphenpenalty=4000
\bibhyphenpenalty=1000

%%%% VERTICAL SPACE IN ALIGNED EQUATIONS

%% Set a global spacing between vertically aligned equaions environments.
%% (To add local space after the break do //[some space ie 12pt])
% \setlength{\jot}{14pt}


%%%% TABLE OF CONTENTS AND LISTS

%% These commands are part of the `tocloft' package.

%% Remove the indent on the list of figures and tables.
\setlength{\cftfigindent}{0pt}
\setlength{\cfttabindent}{0pt}


%% Custom skip before chapters in the TOC. This is useful if, say, the
%% appendicies entry is alone at the foot of the page and you need to 
%% add a little more length.

% \addtolength{\cftbeforechapskip}{2pt}


%% If you don't like capitalised titles in the forematter you can change these
%% here.

% \renewcommand{\listfigurename}{List of figures}
% \renewcommand{\listtablename}{List of tables}

%%%% BIBLIOGRAPHY

%% plus, minus reduces the number of entries which span pages.
\setlength{\bibsep}{2ex plus 1ex minus 1ex}

%% Rename bibliography should you desire
% \renewcommand{\bibname}{References}

%%%% SUBFIGURE CAPTIONS

%% Change size of subfigure captions.
%%\captionsetup[subfloat]{font=normalsize}


%%%% HYPERREF (for hyper package option).

%% Provide options to hyperref. The boolean wrapper
%% makes sure it won't mess up if the hyper option is not used.
\ifthenelse{\boolean{hyperflag}}{%
  \hypersetup{
      plainpages=false,
      breaklinks=true,
      pdftitle={`edengths.cls': The Latex Class File for Formatting
                a Phd Thesis About Clever Stuff at
                The University of Edinburgh},
      pdfauthor={Robert Boberson},
      pdfsubject={Latex Stuff},             % subject of the document
      pdfkeywords={Latex, Thesis Template}, % list of keywords
      colorlinks=true,
%       linkcolor=BrickRed,                   % color of internal links
%       citecolor=Blue,                       % color of links to bibliography
%       filecolor=black,                      % color of file links
%       urlcolor=Violet                       % color of external links
      linkcolor=black,                      % Boring colors. Note, 'black' is
      citecolor=black,                      % blacker than 'Black'.
      filecolor=black,
      urlcolor=black
  }%

  %% \autoref or \Autoref is better to use rather than \ref 
  %% as when using hyperref it links both the title and the number rather 
  %% than just the number.

  %% Create an all uppercase version of autoref, Autoref
  \let\orgautoref\autoref
  \providecommand{\Autoref}
          {\def\equationautorefname{Equation}%
          \def\figureautorefname{Figure}%
          \def\subfigureautorefname{Figure}%
          \def\Itemautorefname{Item}%
          \def\tableautorefname{Table}%
          \def\sectionautorefname{Section}%
          \def\subsectionautorefname{Section}%
          \def\subsubsectionautorefname{Section}%
          \def\chapterautorefname{Chapter}%
          \def\appendixautorefname{Appendix}%
          \def\partautorefname{Part}%
          \orgautoref}
  
  \renewcommand{\autoref}
          {\def\equationautorefname{equation}%
          \def\figureautorefname{figure}%
          \def\subfigureautorefname{figure}%
          \def\Itemautorefname{item}%
          \def\tableautorefname{table}%
          \def\sectionautorefname{section}%
          \def\subsectionautorefname{section}%
          \def\subsubsectionautorefname{section}%
          \def\chapterautorefname{chapter}%
          \def\appendixautorefname{appendix}%
          \def\partautorefname{part}%
          \orgautoref}

  }%
  {}

%%%% FANCY HEADERS (using titlesec)

%% You can mess around with these if you like, but I wouldn't bother, really.
%% DON'T CHANGE THE NAMES 'main' AND 'twomain'.

%% Headers for the main body of the text, ie from the contents onwards.
%% These headers are used when the document is single sided.
%% If there is no chapter number then uppercase lettering is used.
%% Format is {left}{center}{right}. \defaultfont sets the font to sans.
\newpagestyle{main}[\defaultfont\bfseries]{%
  \headrule%
  \sethead%
      {\ifthesection{\toptitlemarks\thesection{.}\space}%
          {\ifthechapter{\thechapter{.}\space}{}}%
       \ifthesection{\toptitlemarks\sectiontitle}%
          {\ifthechapter{\chaptertitle}{\MakeUppercase{\chaptertitle}}}}%
      {}%
      {\thepage}%
  \setfoot%
      {}%
      {}%
      {}%
  }

%% If the twoside option is set, the even pages can have different styles.
%% These are defined in the sqaure brackets [left][centre][right]{}{}{}
%% The headers are now controlled by the twomain pagstyle.
\newpagestyle{twomain}[\defaultfont\bfseries]{%
  \headrule%
  \sethead%
      [\thepage]%
      []%
      [\ifthechapter{\chaptertitle}{\MakeUppercase{\chaptertitle}}]%
      {\ifthesection{\toptitlemarks\thesection{.}\space}%
          {\ifthechapter{\thechapter{.}\space}{}}%
       \ifthesection{\toptitlemarks\sectiontitle}%
          {\ifthechapter{\chaptertitle}{\MakeUppercase{\chaptertitle}}}}%
      {}%
      {\thepage}%
  \setfoot%
      []%
      []%
      []%
      {}%
      {}%
      {}%
  }

%% Redefine the plain page style to use the defaultfont for the
%% numbering.
\renewpagestyle{plain}[\defaultfont]{%
  \sethead%
      {}%
      {}%
      {}%
  \setfoot%
      {}%
      {\thepage}%
      {}%
  }

%%%% FIX VBOX ERROR WITH 'twoside' OPTION

%% Makes all pages the height of the text on that page
\raggedbottom


==> packages.tex <==
%%
%% packages.tex - User defined packages for edengths.tex
%%
%% Copyright (C) 2010-2021 Mathew Topper <damm_horse@yahoo.co.uk>
%%
%%   ABOUT
%%
%% This file contains the user defined packages for a Latex2e template which
%% corresponds to the regulations regarding layout of a thesis submitted within
%% the University of Edinburgh.

%%%% PACKAGES AUTOMATTICALLY PROVIDED BY CLASS 
%%%%
%%%%  (No need to reload.  Options can be provided to these packages using the
%%%%   \PassOptionsToPackage command as per example at end.)

%% ifthen     -   Provides simple boolean commands

%% ifpdf      -   Detects whether pdflatex is being used.

%% graphicx   -   Allows inclusion of graphics in eps or jpg/pdf format

%% geometry   -   A more modern way of setting the page margins.
%%                'report' class options are passed automatically.

%% setspace   -   Define line spacing

%% appendix   -   Required for appendices

%% ae         -   Nicer pdf output using T1 fonts

%% fontenc    -   T1 encoding stops some errors for unknown fonts

%% titlesec   -   Custom chapter titles and page headers

%% caption    -   Custom formatting of captions

%% subcaption -   Use subfigures in captions and formatting of such.

%% tocloft    -   Allow modifications to the table of contents and lists

%% mathptmx   -   Option 'msfonts' to use these alternative font packages.
%% helvet         Note: you could add your own font packages in this file.

%% showlabels -   Print labels on the page if 'labels' option is given.

%% hyperef    -   Put clickable links into the document

%% hypcap     -   Links to figures show the figures rather than just the
%%                caption.

%% nomencl    -   Loaded with option 'nomencl' this provides a ``fly-by-wire''
%%                nomenclature indexing system. See chapter3.tex for an
%%                example.

%% xcolor     -   Loaded with option 'dvipsnames' with provides colors for pdf
%%                output. The options auto adjust for pdflatex and hyperref.
%%                See http://en.wikibooks.org/wiki/LaTeX/Colors for colours.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%          Put ADDITIONAL packages you want to use here           %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Typset URLs properly. This package does automatic breaking of long URLs.
%% If you're using hyperref you dont need this but you might need the
%% 'breakurl' package depending on your compilation route.
%% Note: 'breakurl' must be the last package (which is normally 'hyperref').
\usepackage[hyphens]{url} 

%% AMS Math Packages
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{CJKutf8}

%% Fancy chemical symbols (Might require installation)
% \usepackage[version=3]{mhchem}

%% Better fractions ie 1/2 with diagonal slash
\usepackage{nicefrac}

%% Nicer tables
\usepackage{booktabs}
%% Citations
% \usepackage[natbibapa]{apacite}

%% Proper hyphenation
\usepackage[british]{babel}

%% Rotating
\usepackage{pdflscape}

%% Paragraph control
\usepackage[defaultlines=4,all]{nowidow}

\usepackage{url}
% \usepackage[hidelinks]{hyperref}
\usepackage{amsmath,graphicx}
\usepackage{booktabs}
\usepackage{arydshln}
\usepackage{multirow}
\usepackage{subfigure}
\usepackage{xcolor}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
% \usepackage{hyperref}
\usepackage{subcaption}
\usepackage[ruled, lined, linesnumbered, commentsnumbered, longend]{algorithm2e}
\usepackage{rotating}
% \usepackage{subfig}
\usepackage{hyperref}
% \usepackage{siunitx}
\usepackage[authoryear,round]{natbib}
% \sisetup{
%   detect-all,          % 保持和正文字体一致
%   group-digits = false % 不要千位分隔符
% }

\newcommand{\unit}[2]{#1\,\text{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%             Pass OPTIONS to packages you want here              %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Pass natbib the option 'numbers'
% \PassOptionsToPackage{numbers}{natbib}
% \usepackage[numbers]{natbib}

